MLAE: Masked LoRA Experts for Visual Parameter-Efficient Fine-Tuning

In response to the challenges posed by the extensive parameter updates required for full fine-tuning of large-scale pre-trained models, parameter-efficient fine-tuning (PEFT) methods, exemplified by Low-Rank Adaptation (LoRA), have emerged. LoRA simplifies the fine-tuning process but may still struggle with a certain level of redundancy in low-rank matrices and limited effectiveness from merely increasing their rank. To address these issues, a natural idea is to enhance the independence and diversity of the learning process for the low-rank matrices. Therefore, we propose Masked LoRA Experts (MLAE), an innovative approach that applies the concept of masking to visual PEFT. Our method incorporates a cellular decomposition strategy that transforms a low-rank matrix into independent rank-1 submatrices, or "experts", thus enhancing independence. Additionally, we introduce a binary mask matrix that selectively activates these experts during training to promote more diverse and anisotropic learning, based on expert-level dropout strategies. Our investigations reveal that this selective activation not only enhances performance but also fosters a more diverse acquisition of knowledge with a marked decrease in parameter similarity among MLAE, significantly boosting the quality of the model. Remarkably, MLAE achieves new state-of-the-art (SOTA) performance with an average accuracy score of 78.8% on the VTAB-1k benchmark and 90.9% on the FGVC benchmark, surpassing the previous SOTA result by an average of 0.8% on both benchmarks with approximately half parameters. Our code is available at https://github.com/jie040109/MLAE.

==> table/table_efficiency.tex <==
\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{$\Delta$Param (M) ($\uparrow$)} & \multirow{2}{*}{$\Delta$FLOPs (G) ($\uparrow$)} & \multicolumn{3}{c}{Throughput (imgs/sec)} \\ % \cline{4-6} 
                        &                        &                         & bs=1       & bs=4      & bs=16      \\ \midrule
Full tuning             & 0                      & 0                       & 91.5         & 375.7       & 539.5        \\ \midrule
VPT                     & 0.55                   & 5.6                     & 86.1         & 283.5       & 381.5        \\
Adapter                 & 0.16                   & 0.03                    & 70.9         & 306.6       & 504.7        \\
AdaptFormer             & 0.16                   & 0.03                    & 71.4         & 309.9       & 508.1        \\
NOAH                    & 0.12                   & 0.02                    & 72.1         & 312.7       & 492.9        \\ \midrule
LoRA                    & \multirow{3}{*}{0}     & \multirow{3}{*}{0}      & 91.5         & 375.7       & 539.6        \\
GLoRA                   &                        &                         & 91.5         & 375.7       & 539.6        \\
MLAE                    &                        &                         & 91.5         & 375.2       & 538.5        \\ \bottomrule
\end{tabular}
}
\caption{\textbf{Inference efficiency comparison of MLAE with existing methods during inference.} $\Delta$P and $\Delta$F denote the additional parameters and FLOPs by PEFT methods, respectively. The inference throughput is defined as images per second (imgs/sec). All results are averaged over 100 trials.}
\label{table_efficiency}
\end{table}

